Detecting and Grounding Important Characters in Visual Stories

Characters are essential to the plot of any story. Establishing the characters before writing a story can improve the clarity of the plot and the overall flow of the narrative. However, previous work on visual storytelling tends to focus on detecting objects in images and discovering relationships between them. In this approach, characters are not distinguished from other objects when they are fed into the generation pipeline. The result is a coherent sequence of events rather than a character-centric story. In order to address this limitation, we introduce the VIST-Character dataset, which provides rich character-centric annotations, including visual and textual co-reference chains and importance ratings for characters. Based on this dataset, we propose two new tasks: important character detection and character grounding in visual stories. For both tasks, we develop simple, unsupervised models based on distributional similarity and pre-trained vision-and-language models. Our new dataset, together with these models, can serve as the foundation for subsequent work on analysing and generating stories from a character-centric perspective.

==> 4_experiments.tex <==
\section{Experiments}
\label{experiments}
In this section we will evaluate our model for important character detection and grounding.
For each subtask, we briefly introduce the experimental setting, explain the evaluation metrics, and analyse the results.
% We evaluate the proposed model on the VIST-Character dataset.
\subsection{Character Detection in Text}
We use the spaCy PoS tagger\footnote{https://spacy.io/api/tagger} to obtain the nouns and then identify the characters using WordNet \cite{miller1995wordnet} and obtain co-reference chains using NeuralCoref\footnote{https://github.com/huggingface/neuralcoref}. Table \ref{tab:detc_in_text} shows the results of textual character detection.

\begin{table}[h]
    \centering
    \begin{tabular}{lccc}
    \hline
    Metrics & \begin{tabular}[c]{@{}c@{}}Character\\ Detection\end{tabular} & \begin{tabular}[c]{@{}c@{}}Co-reference\\ Partial Match\end{tabular} & \begin{tabular}[c]{@{}c@{}}Co-reference\\ Exact Match\end{tabular}  \\ \hline
    Precision & 64.7\% & 50.5\% & 35.4\% \\ %\hline
    Recall & 76.0\% & 47.2\% & 28.9\%  \\ \hline
    \end{tabular}%
    \caption{Results for textual character detection and co-reference on VIST-Character.}
    \label{tab:detc_in_text}
\end{table}

\paragraph{Evaluation Metric}
We use precision and recall to evaluate textual character detection and co-reference resolution.
\todo{We should decided whether to use the term "detection" or "identification" (as in Tab. 1) and make this consistent throughout.}
Each character is represented by a co-reference chain.
A ground truth character is successfully identified if the head word of the predicted chain is the same as the head word in the gold-standard chain.
We evaluate the co-reference chains from two perspectives.
Partial match metric computes the the proportion of the correctly detected mentions in the chain on average.
In contrast, exact match implies that the two chains are exactly the same as a whole.

\paragraph{Analysis}
Character detection performance is relatively poor.
Using WordNet and the hypernym method to filter the character words can cause false positive predictions.
For example, \textit{white} is usually used to describe color but, its primary meaning in WordNet is a person name.
Besides, some character words like \textit{great-grandmother} are not included in WordNet.
The partial match score is above 70\% while the exact match is lower than 20\%, which means most co-referred mentions can be successfully detected, but it is difficult to detect the whole chain correctly. The fact that we are working on multi-sentence stories increases the difficulty of co-reference resolution.

\subsection{Character Detection and Clustering in Images}
We compare three methods (1) traditional HOG with SVM-based classifier and feature extraction, (2) pre-trained MTCNN for face detection and Inception ResNet pre-trained on VGGFace2 for computing the face features, and (3) pre-trained MTCNN for face detection and CLIP for face feature extraction. The faces instances are then clustered using k-means to obtain co-reference chains. Table \ref{tab:visual} presents the results of character detection and clustering in images.

\begin{table}[htbp]
\centering
\resizebox{.4\textwidth}{!}{%
\begin{tabular}{lcc}
\hline
Model          &  Detection &  Clustering \\ \hline
% HOG + SVM      & 67.7\%              & 56.6\%               \\ %\hline
MTCNN + ResNet & 69.1\%              & 47.3\%               \\ 
MTCNN + CLIP   & 69.1\%              & 51.3\% \\ \hline
\end{tabular}
}
\caption{Results for visual character detection and clustering. The metrics are recall and matched accuracy respectively. In all cases, k-means is used for clustering.}
\label{tab:visual}
\end{table}

% \begin{table}[h]
%     \centering
%     \begin{tabular}{lccc}
%     \hline
%     Metrics & \begin{tabular}[c]{@{}c@{}}Character\\ Detection\end{tabular} & \begin{tabular}[c]{@{}c@{}}Co-reference\\ Partial Match\end{tabular} & \begin{tabular}[c]{@{}c@{}}Co-reference\\ Exact Match\end{tabular}  \\ \hline
%     Precision & 36.1\% & 74.9\% & 15.6\% \\ %\hline
%     Recall & 44.9\% & 73.2\% & 19.3\%  \\ \hline
%     \end{tabular}%
%     \caption{Results for textual character detection and co-reference on VIST-Character.}
%     \label{tab:detc_in_text}
% \end{table}


\paragraph{Evaluation Metric}
For character detection, a predicted face region is considered as a correct character detection when the bounding box of the face is entirely inside of an annotated body bounding box.
We evaluate character detection using recall rather than precision,
because the images contain many redundant characters in the background, and we only care about the characters that related to the story.

For character clustering task, we use matched accuracy \cite{frank2009evaluating} to evaluate the character clustering performance.
We take the first face in the visual character co-reference chain as its representative head image.
If the head image of a predicted character chain is inside of the ground-truth character's head image, it will be counted as a correct prediction of chain.
Matched accuracy is defined as the percentage of characters with correct category labels. In this project, we use many-to-one accuracy, where each predicted character cluster is matched onto the gold-standard character with the most overlapping instances.
\todo{Why can't we treat the clusters as co-reference chains and evaluate using partial match and exact match, like for textual characters? This would make it more comparable.}

\paragraph{Analysis}
We can observe that MTCNN-based deep neural models perform much better than the traditional HOG-based face detection algorithms.
However, this improvement doesn't have a significant impact on the clustering results.
The reason is that the bottleneck of this pipeline is the clustering algorithm.
The image sequence in the VIST dataset usually contains different angles of the same character, which makes it hard to identify accurate clusters.

\subsection{Character Grounding}
We evaluate distribution similarity-based and CLIP-based alignment applied on the output of the NeuralCoref + MTCNN + CLIP pipeline.
In addition, we report the result of the alignment algorithm on the ground truth input to obtain an estimate of algorithm performance without accumulated error.
The results are shown in Table~\ref{tab:ali}.
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table}[htbp]
% \centering
% \resizebox{.45\textwidth}{!}{%
% \begin{tabular}{|c|c|c|c|}
% \hline
% Input                          & Model              & Recall & Precision \\ \hline
% \multirow{2}{*}{Gold-standard} & Distribution-based & 29.8   & 25.1      \\
%                               & CLIP-based         &        &           \\ \hline
% \multirow{2}{*}{Predictions}   & Distribution-based & 76.4   & 77.5      \\
%                               & CLIP-based         &        &           \\ \hline
% \end{tabular}
% }
% \caption{The performances of the distribution similarity-based alignment algorithm with and without the ground truth annotations as input.}
% \label{tab:ali}
% \end{table}
\begin{table}[htbp]
\centering
\resizebox{.45\textwidth}{!}{%
\begin{tabular}{llcc}
\hline
Input                          & Model              & Recall & Precision \\ \hline
\multirow{2}{*}{Predictions} & Distribution-based & \textbf{29.8\%}   & 25.1\%    \\
                               & CLIP-based         & 23.5\%    & \textbf{26.8\%}          \\ \hline
\multirow{2}{*}{Gold-standard}   & Distribution-based & \textbf{77.5\%}   & -      \\
                               & CLIP-based         &  58.5\%      &  -         \\ \hline
\end{tabular}
}
\caption{Performance of distribution similarity-based and CLIP-based alignment with and without the ground truth annotations as input.}
\label{tab:ali}
\end{table}

\paragraph{Evaluation Metric}
We use recall and precision to evaluate the character grounding task.
Note that recall is preferred to precision in this task, as previous components produce many redundant outputs (e.g., the background characters in images) which depresses the precision score.
Therefore, recall is more accurate and reliable to evaluate how many ground truth alignment relations are successfully retrieved.

\paragraph{Analysis}
We can observe that the accuracy of the distribution-based method with gold standard input reaches 75.7\%.\todo{I think gold standard and prediction are swapped in Tab. 5.}
But the performance when incorporating the detection-and-coreference pipeline is much worse.
This indicates that the alignment algorithm works well, but is very sensitive to errors in the input. The error of previous components accumulate and have a negative impact on the alignment performance.

\subsection{Importance Ranking}

Intuitively, there is a positive relationship between the importance of a character and and its frequency: characters that are central to the plot are mentioned more often than side characters that don't contribute much to the story.

To verify the assumption that character importance is related to frequency, we compute the correlation between the number of occurrences of a character in a story, and the importance rating assigned to that character by the annotators.
We investigate three different settings: (1) input the story text only, (2) input the image sequence only, and (3) input both the image sequence and associated story text. Note that the correlation coefficient is uncomputable when there is only one character or all characters appear equally often in a story, so these instances were removed.

The result is shown in Table \ref{tab:corr} and confirms our hypothesis that character importance is correlated with character frequency.
\todo{I think it would be useful to compute the correlations for both the gold-standard annotation and for the annotation predicted by our best model.}

\begin{table}[h]
\centering
\begin{tabular}{lc}
\hline \text {Story Type} &\text {Correlation Coefficient} \\
\hline
\text{Textual Stories} & 0.61  \\
\text{Visual Stories}  & 0.55  \\
\text{Multi-modal Stories} & 0.62  \\
\hline
\end{tabular}
\caption{Correlation coefficient between the number of occurrences and the importance ranking in different story modalities.}
\label{tab:corr}
\end{table}

We now turn to the most important character in a story, the protagonist. Being able to identify the protagonist is particularly important for story understanding or generation, as the plot revolves around this character. In our setting, the protagonist is expected to be the character with the highest frequency. We can therefore predict the protagonist as the character with the longest co-reference chain. 

We again compare text-only, image-only and multimodal settings, and use the MTCNN + CLIP for the last two. The results are given in Table~\ref{tab:ranking}.

\begin{table}[htbp]
\centering
\begin{tabular}{lccc}
\hline
Model               & Recall@1 & Recall@3 & Recall@5 \\ \hline
Text-only       & 56.4\%    & 86.9\%    & 97.2\%    \\ %\hline
Image-only     & 30.0\%    & 30.8\%    & 31.3\%    \\ %\hline
Multi-modal  & 27.9\%    & 32.4\%    & 37.9\%    \\ \hline
\end{tabular}
\caption{Performance for identifying the most important characters of a story. Recall@1 corresponds to identifying the protagonist. Multi-modal means that both the text and the images of a story are used.}
\label{tab:ranking}
\end{table}

% \begin{table}[h]
% \centering
% \begin{tabular}{cccc}
% \hline
% Model               & Recall @1 & Recall @3 & Recall @5 \\ \hline
% Text Baseline       & 61.0\%    & 34.0\%    & 30.1\%    \\ %\hline
% Visual Baseline     & 30.0\%    & 30.8\%    & 31.3\%    \\ %\hline
% Multi-modal Baseline & 31.2\%    & 37.4\%    & 38.5\%    \\ \hline
% \end{tabular}
% \caption{Performance of importance ranking under different settings.}
% \label{tab:ranking_ground_truth}
% \end{table}

\paragraph{Evaluation Metric}
We use the metric Recall@k to measure performance in predicting the most important characters. Recall@1 corresponds to predicting the protagonist correctly, while Recall@3 or Recall@5 indicate how many of the three or five most important characters have been identified correctly, compared to the human ratings of character importance in VIST-Character.
Note that for the multi-modal model, the recall score is calculated based on the match of multi-modal co-reference chains. Two multi-modal co-reference match if the head
words (first textual mention) are the same.
\todo{These two sentences are unclear to me. Also, why is this a baseline? I've removed the term baseline throughout.}

\paragraph{Analysis}
The text-based model achieves the best performance among the three settings with recall @5 reaching 97.2\%.
The reason is that the story text is treated as the evidence based on which annotators have rated character importance in our dataset. Moreover, the noise in the story text is less than in the image sequence, which makes the text-based importance ranking less error-prone than ranking based on images.

The results of the image-only model are significantly worse, with recall scores of only around 30\%. The reasons are two-fold. Firstly, the performance of the clustering method is not sufficiently high and thus adds a lot of noise to the downstream ranking task.
Secondly, the current evaluation method only considers the head image of the visual character co-reference chain.
Therefore, better clustering methods and more reasonable evaluation methods are needed to improve the image-only setting.
\todo{I don't understand the argument -- isn't the crucial factor the length of the coref chain, as importance is computed based on length? So we need to evaluate using something like exact match, see my earlier comment.}

We can observe that the multi-modal setting performs slightly better than visual setting in terms of Recall@3 and Recall@5.
This means that the injection of textual evidence helps improve the performance of the image-only model somewhat.
From another perspective, the injection of visual evidence degrades the performance of the text-only model as the redundant characters in images bring a lot of noise to the length of the multi-modal co-reference chains if aligned with the wrong textual characters.
\todo{Another interpretation: the injection of visual evidence degrades the performance of the text-only model!}
But we don't think the current method realizes the full potential of the multi-modal model given the large gap between the performance of text-only and multi-modal settings
\todo{We need a better explanation here, and ideally some error analysis.}


\subsection{Plural and Group Characters}

Table~\ref{tab:rank_plu} shows the importance ranking performance for multi-modal input with and without plural and group characters.
We observe that Recall@1 drops by five points with plural and group characters, while Recall@5 increases by about five points.
The reason is that the protagonist is not a plural or group character in most cases.
Therefore, including plural and group nouns makes the most important character prediction more error prone.
However, the top five characters usually contain plural or group characters, thus Recall@5 will be higher when we consider plural and group characters.

\begin{table}[h]
\centering
\begin{tabular}{lcc}
\hline \text { Model } & \text { Recall@1 } & \text { Recall@5 } \\
\hline
\text{Singular Only} & 33.2\% & 32.4\% \\
\text{With Plural/Group} & 27.9\% & 37.9\% \\
\hline
\end{tabular}
\caption{The importance ranking performance of multi-modal input with and without plural and group characters.}
\label{tab:rank_plu}
\end{table}

==> 4_new_experiments.tex <==
\section{Experiments}
\label{experiments}
In this section we will evaluate our model for important character detection and grounding.
For each subtask, we briefly introduce the experimental setting, explain the evaluation metrics, and analyse the results.
% We evaluate the proposed model on the VIST-Character dataset.
\subsection{Character Detection}
For text, we use the spaCy PoS tagger\footnote{https://spacy.io/api/tagger} to obtain the nouns and then identify the characters using WordNet \cite{miller1995wordnet}.
For images, we obtain the faces using pretrained MTCNN \cite{zhang2016joint} and resize them to 160×160.
Table \ref{tab:detc_in_text_and_img} shows the results of character detection.
\begin{table}[h]
    \centering
    \begin{tabular}{lcc}
    \hline
    Modaility      & Precision & Recall \\\hline
    Textual Story  & 74.4\% & 90.2\%  \\
    Image Sequence & 40.5\%  & 69.1\% \\\hline   
    \end{tabular}%
    \caption{Results for character detection in textual story and image sequence on VIST-Character.}
    \label{tab:detc_in_text_and_img}
\end{table}

\paragraph{Evaluation Metric}
We use precision and recall to evaluate textual and visual character detection.
For textual character detection, a predicted character phrase is considered as a correct character detection when the root word of the noun phrase is the same as the gold-standard one.
For visual character detection, a predicted face region is considered as a correct character detection when the bounding box of the face is entirely inside of an annotated body bounding box.


\paragraph{Analysis}
Overall, recall scores are higher than precision scores for both modalities.
The precision of image-based character detection is only 40.5\% and the gap with recall is around 28.6\%.
The reason is that there are a lot of background characters unrelated to the story in the images.
Comparatively, text is less noisy, and we can observe better character detection performance than in images.
However, we found that using WordNet and the hypernym method to filter the character words can cause false positive predictions.
For example, \textit{white} is usually used to describe color but, its primary meaning in WordNet is a person name.
Besides, some character words like \textit{great-grandmother} are not included in WordNet.


\subsection{Character Co-reference}
For textual stories, we obtain co-reference chains using NeuralCoref\footnote{https://github.com/huggingface/neuralcoref}.
For image sequences, we use pre-trained MTCNN for face detection and compare two methods for face feature extraction (1) Inception ResNet pre-trained on VGGFace2 and (2) the pre-trained CLIP model. The face instances are then clustered using k-means to obtain visual co-reference chains. Table \ref{tab:cluster_sim} presents the results of character clustering.

\begin{table}[htbp]
\centering
\begin{tabular}{lcccc}
\hline
\multicolumn{1}{l}{\multirow{2}{*}{Model}} & \multicolumn{2}{c}{Partial Match} & \multicolumn{2}{c}{Exact Match} \\
\multicolumn{1}{c}{} & Precision & Recall & Precision & Recall \\ \hline
NeuralCoref & 50.5\% & 47.2\% & 35.4\% & 28.9\% \\ \hline
ResNet & 34.9\% & 47.3\% & 10.7\% & 17.5\% \\
CLIP & 35.8\% & 51.3\% & 25.8\% & 23.8\% \\ \hline
\end{tabular}
\caption{Results for character co-reference. For NeuralCoref, the input is the character mentions detected by PoS + WordNet. For the visual models, face instances are obtained by MTCNN and k-means is used for clustering.}
\label{tab:cluster_sim}
\end{table}

% \begin{table*}[htbp]
% \centering
% \begin{tabular}{llcccc}
% \hline
% \multicolumn{1}{l}{\multirow{2}{*}{Modality}} & \multicolumn{1}{l}{\multirow{2}{*}{Model}} & \multicolumn{2}{c}{Partial Match} & \multicolumn{2}{c}{Exact Match} \\
% \multicolumn{1}{l}{} & \multicolumn{1}{c}{} & Precision & Recall & Precision & Recall \\ \hline
% Textual Story & NeuralCoref & 50.5\% & 47.2\% & 35.4\% & 28.9\% \\ \hline
% \multirow{2}{*}{Image Sequence} & MTCNN + ResNet & 34.9\% & 47.3\% & 10.7\% & 17.5\% \\
%  & MTCNN + CLIP & 35.8\% & 51.3\% & 25.8\% & 23.8\% \\ \hline
% \end{tabular}
% \caption{Results for character clustering. For the visual models, k-means is used for clustering.}
% \label{tab:cluster}
% \end{table*}


\paragraph{Evaluation Metric}
Each character is represented by a co-reference chain and matched onto the gold-standard co-reference chain with the most overlapping instances.
We evaluate the co-reference chains from two perspectives.
Partial match computes the the percentage of the correctly detected mentions in the chain.
In contrast, exact match requires that the two chains are exactly the same.
We report recall and precision scores for both metrics.


\paragraph{Analysis}
% \textbf{visual}
% We can observe that MTCNN-based deep neural models perform much better than the traditional HOG-based face detection algorithms.
% However, this improvement doesn't have a significant impact on the clustering results.

% first partial vs. exact
In general, partial match scores are higher than exact match, which means that co-referred mentions can be successfully detected, but it is difficult to detect the whole chain correctly. The reasons are twofold. First, the fact that we are working on multi-sentence stories increases the difficulty of textual co-reference resolution.
Second, the image sequence in the VIST dataset usually contains different angles of the same character, which makes it hard to identify exactly accurate clusters.

% then text vs. image
As we compare the performance on different modalities, we can observe that clustering in text performs better than in images.
Especially in terms of the the exact match, textual character clustering can reach 35.4\% precision, which is around 10\% higher than visual character clustering because of the redundant characters detected in images.

%CLIP vs. ResNet
For the visual models, we can observe that CLIP-based clustering consistently outperforms ResNet-based clustering.
% There are two reasons for this.
% First, Inception ResNet is pretrained on VGGFace2 that contains only 3.31 million labelled images, while CLIP is pretrained on 400 million images with captions.
% So CLIP can learn better image features and can generalise better.
CLIP is explicitly pretrained on matching tasks, using dot products to compute similarity, which is related to Euclidean distance used by the downstream K-means algorithm.

\subsection{Character Grounding}
We evaluate distributional similarity-based and CLIP-based alignment applied on the output of the NeuralCoref and MTCNN + CLIP pipelines.
In addition, we report the result of the alignment algorithm on gold standard input to obtain an estimate of algorithm performance without accumulated error.
The results are shown in Table~\ref{tab:ali}.
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table}[htbp]
% \centering
% \resizebox{.45\textwidth}{!}{%
% \begin{tabular}{|c|c|c|c|}
% \hline
% Input                          & Model              & Recall & Precision \\ \hline
% \multirow{2}{*}{Gold-standard} & Distribution-based & 29.8   & 25.1      \\
%                               & CLIP-based         &        &           \\ \hline
% \multirow{2}{*}{Predictions}   & Distribution-based & 76.4   & 77.5      \\
%                               & CLIP-based         &        &           \\ \hline
% \end{tabular}
% }
% \caption{The performances of the distribution similarity-based alignment algorithm with and without the ground truth annotations as input.}
% \label{tab:ali}
% \end{table}
\begin{table}[htbp]
\centering
\resizebox{.45\textwidth}{!}{%
\begin{tabular}{llcc}
\hline
Input                          & Model              & Recall & Precision \\ \hline
\multirow{2}{*}{Predictions} & Distribution-based & \textbf{29.8\%}   & 25.1\%    \\
                               & CLIP-based         & 23.5\%    & \textbf{26.8\%}          \\ \hline
\multirow{2}{*}{Gold-standard}   & Distribution-based & \textbf{77.5\%}   & -      \\
                               & CLIP-based         &  58.5\%      &  -         \\ \hline
\end{tabular}
}
\caption{Performance of distribution similarity-based and CLIP-based alignment with and without the gold standard annotations as input. Best results are highlighted in bold..}
\label{tab:ali}
\end{table}

\paragraph{Evaluation Metric}
We use recall and precision to evaluate the character grounding task.
Note that recall is preferred to precision in this task, as previous components produce many redundant outputs (e.g., the background characters in images) which depresses the precision score.

\paragraph{Analysis}
% We can observe that the accuracy of the distribution-based method with gold standard input reaches 77.5\%.

% first gold-standard vs. predictions
We can observe that the performance is much better with gold-standard input than when detection-and-coreference is used.
This indicates that the alignment algorithm works well, but is very sensitive to errors in the input. The error of previous components accumulate and have a negative impact on the alignment performance.

% CLIP vs. distribution
Interestingly, CLIP does not outperform the distribution-based model.
The reason is that CLIP is pretrained on image-caption pairs whose the caption is usually specific and detailed.
However, the VIST stories contain many generic words (e.g., \textit{he}, \textit{boy}) that appear frequently in the textual co-reference chains, making it difficult for CLIP to predict the alignment relation.

\subsection{Importance Ranking}

Intuitively, there is a positive relationship between the importance of a character and and its frequency: characters that are central to the plot are mentioned more often than side characters that don't contribute much to the story.

To verify the assumption that character importance is related to frequency, we compute the correlation between the number of occurrences of a character in a story (i.e., the length of gold-standard co-reference chain), and the importance rating assigned to that character by the annotators.
Specifically, we investigate the correlation between a character's importance rating and (1) the number of occurrences in story text only, (2) the number of occurrences in image sequence only, and (3) the number of occurrences in both the image sequence and associated story text. Note that the correlation coefficient is uncomputable when there is only one character or all characters appear equally often in a story, so these instances were removed.
The result is shown in Table \ref{tab:corr} and confirms our hypothesis that character importance is correlated with character frequency.

\begin{table}[h]
\centering
\begin{tabular}{lc}
\hline \text {Story Type} &\text {Correlation Coefficient} \\
\hline
\text{Textual Stories} & 0.61  \\
\text{Visual Stories}  & 0.55  \\
\text{Multi-modal Stories} & 0.62  \\
\hline
\end{tabular}
\caption{Correlation coefficient between the number of occurrences and the importance ranking in different story modalities in the gold-standard VIST-Character dataset.}
\label{tab:corr}
\end{table}

We now turn to the most important character in a story, the protagonist. Being able to identify the protagonist is particularly important for story understanding or generation, as the plot revolves around this character. In our setting, the protagonist is expected to be the character with the highest frequency. We can therefore predict the protagonist as the character with the longest co-reference chain. 

We again compare text-only, image-only and multimodal settings, and use MTCNN + CLIP for the last two. The results are given in Table~\ref{tab:ranking}.

\begin{table}[htbp]
\centering
\begin{tabular}{lccc}
\hline
Model               & P@1 & P@3 & P@5 \\ \hline
Text-only       & 56.4\%    & 86.9\%    & 97.2\%    \\ %\hline
Image-only     & 30.0\%    & 30.8\%    & 31.3\%    \\ %\hline
Multi-modal  & 27.9\%    & 32.4\%    & 37.9\%    \\ \hline
\end{tabular}
\caption{Performance for identifying the most important characters of a story. P@k means Precision@k. P@1 corresponds to identifying the protagonist. Multi-modal means that both the text and the images of a story are used.}
\label{tab:ranking}
\end{table}


\paragraph{Evaluation Metric}
We use the metric Precision@k to measure performance in predicting the most important characters. Precision@1 corresponds to predicting the protagonist correctly, while Precision@3 or Precision@5 indicate how many of the three or five most important characters have been identified correctly, compared to the human ratings of character importance in our VIST-Character dataset.
Note that for the multi-modal model, the precision score is calculated based on the match of multi-modal co-reference chains. Two multi-modal co-reference match if the head words (first textual mention) are the same.

\paragraph{Analysis}
The text-based model achieves the best performance among the three settings with Precision@5 reaching 97.2\%.
The reason is that the story text is treated as the evidence based on which annotators have rated character importance in our dataset. Moreover, the noise in the story text is less than in the image sequence, which makes the text-based importance ranking less error-prone than ranking based on images.

The results of the image-only model are significantly worse, with precision scores of only around 30\%. The reasons are two-fold. Firstly, the performance of clustering for co-reference resolution is not sufficiently high and thus adds a lot of noise to the downstream ranking task.
Secondly, the current evaluation method only considers the head image of the visual character co-reference chain.
Therefore, better co-reference resolution methods and more reasonable evaluation methods are needed to improve the image-only setting.

We can observe that the multi-modal setting performs slightly better than visual setting in terms of Precision@3 and Precision@5.
This means that the injection of textual evidence helps improve the performance of the image-only model somewhat.
From another perspective, the injection of visual evidence degrades the performance of the text-only model as the redundant characters in images bring a lot of noise to the length of the multi-modal co-reference chains if aligned with the wrong textual characters.
But we don't think the current method realizes the full potential of the multi-modal model given the large gap between the performance of text-only and multi-modal settings


\subsection{Plural and Group Characters}
\begin{table}[]
\centering
\begin{tabular}{lcccc}
\hline
\multirow{2}{*}{Input} & \multicolumn{2}{c}{Grounding} & \multicolumn{2}{c}{Ranking} \\
                       & Precision       & Recall      & P@1     & P@5     \\ \hline
Singular          & 23.7\%          & 34.2\%      & 33.2\%       & 32.4\%       \\
Plural            & 50.8\%          & 17.4\%      & -            & -            \\ \hline
Both                   & 29.8\%          & 25.1\%      & 27.9\%       & 37.9\%       \\ \hline
\end{tabular}
\caption{The character grounding and importance ranking performance of multi-modal input with and without plural and group characters. P@k means Precision@k.}
\label{tab:rank_pl}
\end{table}

Table~\ref{tab:rank_pl} shows the character grounding and importance ranking performance for multi-modal input with and without plural and group characters.
For character grounding, the precision of plural and group characters reaches 50.8\% while the recall is only 17.4\%.
The reason our grounding algorithm sets a high threshold (i.e., 0.6) for linking a visual character to a plural or group textual character.
This threshold prevents the model from overpredicting plural characters, given that these are relatively rare in the VIST stories.

For important ranking, we observe that Precision@1 drops by five points with plural and group characters, while Precision@5 increases by about five points.
The reason is that the protagonist is not a plural or group character in most cases.
Therefore, including plural and group nouns makes the most important character prediction more error prone.
However, the top five characters usually contain plural or group characters, thus Precision@5 will be higher when we consider plural and group characters.



==> 4_spanbert_experiments.tex <==
\section{Experiments}
\label{experiments}
In this section we will evaluate our model for important character detection and grounding.
For each subtask, we briefly introduce the experimental setting, explain the evaluation metrics, and analyse the results.
% We evaluate the proposed model on the VIST-Character dataset.

\subsection{Character Detection}
We use the spaCy PoS tagger (https://spacy.io/api/tagger) to obtain the nouns in text and then identify the characters using WordNet \cite{miller1995wordnet}.
For images, we obtain the faces using MTCNN \cite{zhang2016joint} and resize them to 160×160.
Table \ref{tab:detc_in_text_and_img} shows the results of character detection.

\begin{table}[t]
    \centering
    \begin{tabular}{lcc}
    \hline
    Modaility      & Precision & Recall \\\hline
    Textual Story  & 74.4\% & 90.3\%  \\
    Image Sequence & 40.5\%  & 69.1\% \\\hline   
    \end{tabular}%
    \caption{Results for character detection in textual story and image sequence on VIST-Character.}
    \label{tab:detc_in_text_and_img}
\end{table}

\paragraph{Evaluation Metric}
We use precision and recall to evaluate textual and visual character detection.
For textual character detection, a predicted character phrase is considered as a correct character detection when the head word of the noun phrase is the same as the gold-standard one.
For visual character detection, a predicted face region is considered as a correct character detection when the bounding box of the face is entirely inside of an annotated body bounding box.

\paragraph{Analysis}
Overall, recall scores are higher than precision scores for both modalities.
The precision of image-based character detection is only 40.5\% and the gap with recall is around 28.6\%.
The reason is that there are a lot of background characters unrelated to the story in the images.
Comparatively, text is less noisy, and we can observe better character detection performance than in images.
However, we found that using WordNet and the hypernym method to filter the character words can cause false positive predictions.
For example, \textit{white} is usually used to describe color but, its primary meaning in WordNet is a person name.
Besides, some character words like \textit{great-grandmother} are not included in WordNet.

\subsection{Character Co-reference}
For textual stories, we experiment with two different approaches to obtain co-reference chains (1) NeuralCoref \cite{clark2016improving} and (2) SpanBERT \cite{joshi2020spanbert}.
For image sequences, we use pre-trained MTCNN for face detection and compare two methods for face feature extraction (1) Inception ResNet pre-trained on VGGFace2 and (2) the pre-trained CLIP model. The face instances are then clustered using k-means to obtain visual co-reference chains. Table \ref{tab:cluster_sim} presents the character co-reference results for both modalities.

\begin{table}[t]
\centering
\begin{tabular}{lcccc}
\hline
\multicolumn{1}{l}{\multirow{2}{*}{Model}} & \multicolumn{2}{c}{Partial Match} & \multicolumn{2}{c}{Exact Match} \\
\multicolumn{1}{c}{} & Precision & Recall & Precision & Recall \\ \hline
NeuralCoref & \textbf{49.3\%} & 48.6\% & 29.2\% & 32.4\% \\ 
SpanBERT & 48.0\% & \textbf{51.1\%} & \textbf{30.0\%} &  \textbf{33.2}\%\\ \hline
ResNet & 34.9\% & 47.3\% & 10.7\% & 17.5\% \\
CLIP & \textbf{35.8\%} & \textbf{51.3\%} & \textbf{25.8\%} & \textbf{23.8\%} \\ \hline
\end{tabular}
\caption{Results for character co-reference. For the textual models, the input is the character mentions detected by PoS + WordNet. For the visual models, face instances are obtained by MTCNN and k-means is used for clustering.}
\label{tab:cluster_sim}
\end{table}

% \begin{table*}[htbp]
% \centering
% \begin{tabular}{llcccc}
% \hline
% \multicolumn{1}{l}{\multirow{2}{*}{Modality}} & \multicolumn{1}{l}{\multirow{2}{*}{Model}} & \multicolumn{2}{c}{Partial Match} & \multicolumn{2}{c}{Exact Match} \\
% \multicolumn{1}{l}{} & \multicolumn{1}{c}{} & Precision & Recall & Precision & Recall \\ \hline
% Textual Story & NeuralCoref & 50.5\% & 47.2\% & 35.4\% & 28.9\% \\ \hline
% \multirow{2}{*}{Image Sequence} & MTCNN + ResNet & 34.9\% & 47.3\% & 10.7\% & 17.5\% \\
%  & MTCNN + CLIP & 35.8\% & 51.3\% & 25.8\% & 23.8\% \\ \hline
% \end{tabular}
% \caption{Results for character clustering. For the visual models, k-means is used for clustering.}
% \label{tab:cluster}
% \end{table*}


\paragraph{Evaluation Metric}
Each character is represented by a co-reference chain and matched onto the gold-standard co-reference chain with the most overlapping mentions.
We evaluate the co-reference chains from two perspectives.
Partial match computes the the percentage of the correctly detected mentions in the chain.
In contrast, exact match requires that the two chains are exactly the same.
We report recall and precision for both metrics.


\paragraph{Analysis}
% \textbf{visual}
% We can observe that MTCNN-based deep neural models perform much better than the traditional HOG-based face detection algorithms.
% However, this improvement doesn't have a significant impact on the clustering results.

% first partial vs. exact
In general, partial match scores are higher than exact match, which means that co-referred mentions can be successfully detected, but it is difficult to detect the whole chain correctly. The reasons are twofold. First, the fact that we are working on multi-sentence stories increases the difficulty of textual co-reference resolution.
Second, the image sequences in the VIST dataset usually contain different views of the same character, which makes it hard to form accurate clusters.

% then text vs. image
Comparing modalities, we observe that clustering in text performs better than in images across the board, with the exception of recall for partial match. We attribute this to the redundant characters detected in images, i.e., characters that are depicted but do not play a role in the story (e.g., people in the background).

For text-based models, SpanBERT outperforms NeuralCoref in most metrics, while for visual models, CLIP consistently outperforms ResNet. In further experiments, we will use SpanBERT and CLIP, respectively.
% There are two reasons for this.
% First, Inception ResNet is pretrained on VGGFace2 that contains only 3.31 million labelled images, while CLIP is pretrained on 400 million images with captions.
% So CLIP can learn better image features and can generalise better.

\subsection{Character Grounding}
We evaluate distributional similarity-based and CLIP-based alignment applied on the output of the SpanBERT and MTCNN + CLIP pipelines.
In addition, we report the result of the alignment algorithm on gold standard input to obtain an estimate of its performance without accumulated error.
The results are shown in Table~\ref{tab:ali}.
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table}[htbp]
% \centering
% \resizebox{.45\textwidth}{!}{%
% \begin{tabular}{|c|c|c|c|}
% \hline
% Input                          & Model              & Recall & Precision \\ \hline
% \multirow{2}{*}{Gold-standard} & Distribution-based & 29.8   & 25.1      \\
%                               & CLIP-based         &        &           \\ \hline
% \multirow{2}{*}{Predictions}   & Distribution-based & 76.4   & 77.5      \\
%                               & CLIP-based         &        &           \\ \hline
% \end{tabular}
% }
% \caption{The performances of the distribution similarity-based alignment algorithm with and without the ground truth annotations as input.}
% \label{tab:ali}
% \end{table}
\begin{table}[t]
\centering
\resizebox{.45\textwidth}{!}{%
\begin{tabular}{llcc}
\hline
Input                          & Model              & Recall & Precision \\ \hline
\multirow{2}{*}{Predictions} & Distribution-based & \textbf{27.3\%}   & 27.5\%    \\
                               & CLIP-based         & 21.7\%    & \textbf{28.5\%}          \\ \hline
\multirow{2}{*}{Gold-standard}   & Distribution-based & \textbf{77.5\%}   & -      \\
                               & CLIP-based         &  58.5\%      &  -         \\ \hline
\end{tabular}
}
\caption{Performance of distribution similarity-based and CLIP-based alignment with and without the gold standard annotations as input. Best results are highlighted in bold.}
\label{tab:ali}
\end{table}

\paragraph{Evaluation Metric}
We use recall and precision to evaluate the character grounding task.
Note that recall is preferred to precision in this task, as visual character detection returns redundant characters (see above), which depresses the precision score.

\paragraph{Analysis}
% We can observe that the accuracy of the distribution-based method with gold standard input reaches 77.5\%.

% first gold-standard vs. predictions
We can observe that the performance is much better with gold-standard input than when detection-and-coreference is used.
This indicates that the alignment algorithm works well, but is very sensitive to errors in the input. The errors of previous components accumulate and have a negative impact on the alignment performance.

% CLIP vs. distribution
Interestingly, CLIP does not outperform the distribution-based model.
The reason is that CLIP is pretrained on image-caption pairs whose the caption is usually specific and detailed.
However, the VIST stories contain many generic words (e.g., \textit{he}, \textit{boy}) that appear frequently in the textual co-reference chains, making it difficult for CLIP to predict the alignment relation.
More detail on the CLIP-based grounding results are provided in the supplementary material.

\subsection{Importance Ranking}

Intuitively, there is a positive relationship between the importance of a character and and its frequency: characters that are central to the plot are mentioned more often than side characters that don't contribute much to the story.

To verify the assumption that character importance is related to frequency, we compute the Pearson's correlation between the number of occurrences of a character in a story (i.e., the length of gold-standard co-reference chain), and the importance rating assigned to that character by the annotators.
Specifically, we investigate the correlation between a character's importance rating and (1) the number of occurrences in story text only, (2) the number of occurrences in image sequence only, and (3) the number of occurrences in both the image sequence and associated story text. Note that the correlation coefficient is uncomputable when there is only one character or all characters appear equally often in a story, so these instances were removed.
The result is shown in Table \ref{tab:corr} and confirms our hypothesis that character importance is correlated with character frequency.

\begin{table}[h]
\centering
\begin{tabular}{lc}
\hline \text {Story Type} &\text {Pearson's Correlation} \\
\hline
\text{Textual Stories} & 0.61  \\
\text{Visual Stories}  & 0.55  \\
\text{Multi-modal Stories} & 0.62  \\
\hline
\end{tabular}
\caption{Pearson's correlation between the number of occurrences and the importance ranking in different story modalities in the gold-standard VIST-Character dataset.}
\label{tab:corr}
\end{table}

We now turn to the most important character in a story, the protagonist. Being able to identify the protagonist is particularly important for story understanding or generation, as the plot revolves around this character. In our setting, the protagonist is expected to be the character with the highest frequency. We can therefore predict the protagonist as the character with the longest co-reference chain. 

We again compare text-only, image-only and multimodal settings, and use MTCNN + CLIP for the last two. The results are given in Table~\ref{tab:ranking}.

\begin{table}[t]
\centering
\begin{tabular}{lccc}
\hline
Model               & P@1 & P@3 & P@5 \\ \hline
Text-only       & 53.6\%    & 79.2\%    & 87.4\%    \\ %\hline
Image-only     & 30.0\%    & 30.8\%    & 31.3\%    \\ %\hline
Multi-modal  & 29.4\%    & 34.7\%    & 34.3\%    \\ \hline
\end{tabular}
\caption{Performance for identifying the most important characters of a story. P@k means Precision@k. P@1 corresponds to identifying the protagonist. Multi-modal means that both the text and the images of a story are used.}
\label{tab:ranking}
\end{table}

\paragraph{Evaluation Metric}
We use the metric Precision@k to measure performance in predicting the most important characters. Precision@1 corresponds to predicting the protagonist correctly, while Precision@3 or Precision@5 indicate how many of the three or five most important characters have been identified correctly, compared to the human ratings of character importance in our VIST-Character dataset.
Note that for the multi-modal model, the precision score is calculated based on the match of multi-modal co-reference chains. Two multi-modal co-reference match if the head words (first textual mention) are the same.

\paragraph{Analysis}
The text-based model achieves the best performance among the three settings with Precision@5 reaching 87.4\%.
The reason is that the story text is treated as the evidence based on which annotators have rated character importance in our dataset. Moreover, the noise in the story text is less than in the image sequence, which makes the text-based importance ranking less error-prone than ranking based on images.

The results of the image-only model are significantly worse, with precision scores of only around 30\%. The reasons are two-fold. Firstly, the performance of clustering for co-reference resolution is not sufficiently high and thus adds a lot of noise to the downstream ranking task.
Secondly, the current evaluation method only considers the head image of the visual character co-reference chain.
Therefore, better co-reference resolution methods and more reasonable evaluation methods are needed to improve the image-only setting.

We can observe that the multi-modal setting performs slightly better than visual setting in terms of Precision@3 and Precision@5.
This means that the injection of textual evidence helps improve the performance of the image-only model somewhat.
From another perspective, the injection of visual evidence degrades the performance of the text-only model as the redundant characters in images bring a lot of noise to the length of the multi-modal co-reference chains if aligned with the wrong textual characters.
But we don't think the current method realizes the full potential of the multi-modal model given the large gap between the performance of text-only and multi-modal settings.

\subsection{Plural and Group Characters}
\begin{table}[]
\centering
\begin{tabular}{lcccc}
\hline
\multirow{2}{*}{Input} & \multicolumn{2}{c}{Grounding} & \multicolumn{2}{c}{Ranking} \\
                       & Precision       & Recall      & P@1     & P@5     \\ \hline
Singular          & 34.5\%          & 21.5\%      & 33.2\%       & 32.4\%       \\
Plural            & 20.9\%          & 47.5\%      & -            & -            \\ \hline
Both                   & 27.3\%          & 27.5\%      & 27.9\%       & 37.9\%       \\ \hline
\end{tabular}
\caption{The character grounding and importance ranking performance of multi-modal input with and without plural and group characters. P@k means Precision@k.}
\label{tab:rank_pl}
\end{table}

Table~\ref{tab:rank_pl} shows the character grounding and importance ranking performance for multi-modal input with and without plural and group characters.
For character grounding, the precision of plural and group characters reaches 47.5\% while the recall is only 20.9\%.
The reason our grounding algorithm sets a high threshold (i.e., 0.6) for linking a visual character to a plural or group textual character.
This threshold prevents the model from overpredicting plural characters, given that these are relatively rare in the VIST stories.

For important ranking, we observe that Precision@1 drops by five points with plural and group characters, while Precision@5 increases by about five points.
The reason is that the protagonist is not a plural or group character in most cases.
Therefore, including plural and group nouns makes the most important character prediction more error prone.
However, the top five characters usually contain plural or group characters, thus Precision@5 will be higher when we consider plural and group characters.


